Evaluating and Modeling Attribution for Cross-Lingual Question Answering

Trustworthy answer content is abundant in many high-resource languages and is instantly accessible through question answering systems, yet this content can be hard to access for those that do not speak these languages. The leap forward in cross-lingual modeling quality offered by generative language models offers much promise, yet their raw generations often fall short in factuality. To improve trustworthiness in these systems, a promising direction is to attribute the answer to a retrieved source, possibly in a content-rich language different from the query. Our work is the first to study attribution for cross-lingual question answering. First, we collect data in 5 languages to assess the attribution level of a state-of-the-art cross-lingual QA system. To our surprise, we find that a substantial portion of the answers is not attributable to any retrieved passages (up to 50% of answers exactly matching a gold reference) despite the system being able to attend directly to the retrieved text. Second, to address this poor attribution level, we experiment with a wide range of attribution detection techniques. We find that Natural Language Inference models and PaLM 2 fine-tuned on a very small amount of attribution data can accurately detect attribution. Based on these models, we improve the attribution level of a cross-lingual question-answering system. Overall, we show that current academic generative cross-lingual QA systems have substantial shortcomings in attribution and we build tooling to mitigate these issues.

==> tables/attribution_of_cora_full_details_in_lang.tex <==

\begin{table*}
\centering%
\renewcommand*{\arraystretch}{.9}
\begin{tabu}{l c c c c }%
	\toprule
	\textbf{Query Language}&  \textbf{Passage Language} &  \%  \bf AIS &  \bf \% AIS of EM & \bf \% AIS of non-EM \\ %
	\midrule

 

\textsc{bn} & \textsc{bn} & 25.0 / 40.2 & 41.8 / 65.5 & 22.3 / 36.1 \\
\textsc{bn} & \textsc{en} & 2.3 / 3.3 & 0.0 / 0.0 & 2.6 / 3.8 \\
\textsc{bn} & \textsc{any} & 27.5 / 44.2 & 41.8 / 67.3 & 25.2 / 40.5 \\
\hdashline
\textsc{fi} & \textsc{fi} & 36.5 / 46.0 & 64.3 / 75.0 & 25.7 / 34.7 \\
\textsc{fi} & \textsc{en} & 1.0 / 4.00 & 3.6 / 5.36 & 0.0 / 3.47 \\

\textsc{fi} & \textsc{any} & 38.5 / 51.0 & 67.9 / 80.4 & 27.1 / 39.6 \\
\hdashline
\textsc{ja} & \textsc{ja} & 13.0 / 30.8 & 22.4 / 51.0 & 8.2 / 20.6 \\
\textsc{ja} & \textsc{en} & 0.0 / 2.05 & 0.0 / 0.0 & 0.0 / 3.1 \\

\textsc{ja} & \textsc{any} & 13.0 / 33.6 & 22.4 / 53.1 & 8.2 / 23.7 \\
\hdashline
\textsc{ru} & \textsc{ru} & 28.1 / 43.2 & 45.0 / 67.5 & 23.4 / 36.6 \\
\textsc{ru} & \textsc{en} & 1.1 / 1.1 & 0.0 / 0.0 & 1.4 / 1.4 \\

\textsc{ru} & \textsc{any} & 29.2 / 44.3 & 45.0 / 67.5 & 24.8 / 37.9 \\
\hdashline
\textsc{te} & \textsc{te} & 23.2 / 32.2 & 69.0 / 93.1 & 13.2 / 18.9 \\
\textsc{te} & \textsc{en}    & 0.3 / 0.3 & 1.7 / 0.0 & 0.0 / 0.38 \\

\textsc{te} & \textsc{any} & 23.8 / 32.5 & 72.4 / 93.1 & 13.2 / 19.2 \\

\bottomrule
\end{tabu}
\caption{
Percentage of attributed answers (\%~AIS) to the \textsc{top-1} / \textsc{All} passages fed to \mGen. We report the \textbf{\%AIS} on XOR-TyDiQA validation split. 
\textbf{\%~AIS of EM} corresponds to the percentage of attributable answers among the Exact-Matched answers. 
\textbf{\%~AIS of non-EM} corresponds to the percentage of attributable answers among the non-Exact-Matched answers (i.e. that differ from the gold answer). We also report the attribution-level considering only the English passages as our candidates (with ``Passage Language'' column equals to \textsc{En}), only the in-language passages (with ``Passage Language'' column equals to ``Query Language'') as our candidates. 
}%
\label{tab:ais_em_non_em}
\vspace{-1em}
\end{table*}


==> tables/slides.tex <==

\begin{table}[t!]
\centering\footnotesize
\begin{tabular}{*{5}{>{\centering\arraybackslash}p{1cm}}}

	\toprule
	
	\multicolumn{5}{c}{\bf \textbf{ \% Attributable predictions (AIS)}} \\
subset & \bf \textsc{bn} & \bf \textsc{fi} & \bf \textsc{ja} & \bf \textsc{ru} & \bf\textsc{te} \\
	\midrule
 EM & 67.3 & 80.4 & 53.1 & 67.5 & 93.1\\

\bottomrule
\end{tabular}
\caption{\% of answers exactly-matching the gold answer attributed to at least one passage fed to the \textsc{mGen}.  
}%
\label{tab:attribution_cora_larger_sample}
\end{table}
